ArtiFix: Localizing and Repairing Artifacts in AI-Generated Videos

AI-generated videos may appear realistic, but an occasional local artifact, such as an extra finger or two, can ruin the entire result. Iteratively regenerating the entire video incurs the full generation cost and risks changing content that was already correct. We introduce ArtiFix, an automatic pipeline that repairs such artifacts from the video alone and leaves every pixel outside the repair region unchanged. A lightweight video localizer identifies the region containing the artifact, and a video inpainting model reconstructs the masked region, conditioned on the surrounding video and a reference cutout of the original object to preserve its identity. Additionally, the computational cost of artifact inpainting scales with the size of the repair region rather than the full video. We further refine this inpainter through preference tuning on its own samples, ranked by a Video Jev video realism model, improving the observer-rated repair quality without a detected loss in preservation. Because current automated metrics do not reliably capture artifact removal, we evaluate repairs through a perceptual study. Observers rank ArtiFix highest in both artifact removal and original video preservation.

==> figures/fig_fix_vs_preserve.tex <==
% Graphic in figures/assets/, made by the study session (rating-app paper_figs.py).
\begin{figure}[t]
\centering
\IfFileExists{figures/assets/fig_fix_vs_preserve.pdf}{\includegraphics[width=0.72\linewidth]{figures/assets/fig_fix_vs_preserve.pdf}}%
{\TODO{upload figures/assets/fig\_fix\_vs\_preserve.pdf (rating-app/analysis\_out/paper/) to Overleaf}}
% \caption{How well each inpainting method fixes the artifact (x) against how well it preserves the video (y), as
% MOS recovered with SUREAL from eleven observers on a 5-point scale. Circles edit only a region and squares regenerate the
% whole video. \method and the same pipeline without preference tuning are the only methods rated well on both, while the
% open regenerators and EditCtrl fall into the lower left. The pipeline without the reference cut-out is shown in
% the supplementary material. Gemini Omni 1.1 Flash removes
% artifacts about as well as \method but preserves the video less. Error bars are 95\% confidence intervals from a
% two-level bootstrap over observers and clips.}
\caption{Fixing (x) against preservation (y) per method, SUREAL MOS from eleven observers with 95\% confidence intervals. Circles edit a region and squares regenerate the video. Only \method and its untuned version are rated well on both, and Gemini Omni 1.1 Flash preserves the video less than \method.}
\label{fig:fixpreserve}
\end{figure}


==> figures/fig_mos_rows_inpainting.tex <==
% Graphic in figures/assets/, made by the study session (rating-app paper_figs.py).
\begin{figure*}[t]
\centering
\IfFileExists{figures/assets/fig_mos_rows_inpainting.pdf}{\includegraphics[width=0.85\textwidth]{figures/assets/fig_mos_rows_inpainting.pdf}}%
{\TODO{upload figures/assets/fig\_mos\_rows\_inpainting.pdf to Overleaf}}
\caption{Ratings of six of the seven inpainting conditions, all on the region of our localizer (the pipeline without the
reference cut-out is shown in the supplementary material), for how well the artifact
is fixed (left) and how well the video is preserved (right). A dot is one clip, and black marks the mean with its 95\%
confidence interval (SUREAL MOS from eleven observers, bootstrap over observers and clips). \method is rated highest on
both statements, and the spread of the dots shows that Gemini Omni 1.1 Flash varies far more from clip to clip than
\method. $^*$ differs from \method without preference tuning and $^\dagger$ from \method (Wilcoxon signed-rank test
over clips, Holm-corrected, $p<.05$).}
\label{fig:mosinp}
\end{figure*}


==> figures/fig_mos_rows_localization.tex <==
% Graphic in figures/assets/, made by the study session (rating-app paper_figs.py). \input in the Localization paragraph
% of sec/4b_study.tex. Pairs with figures/assets/fig_mos_rows_inpainting.pdf (inpainting conditions, fixed / preserved).
\begin{figure*}[t]
\centering
\IfFileExists{figures/assets/fig_mos_rows_localization.pdf}{\includegraphics[width=0.72\textwidth]{figures/assets/fig_mos_rows_localization.pdf}}%
{\TODO{upload figures/assets/fig\_mos\_rows\_localization.pdf to Overleaf}}
% \caption{Ratings of the three localizations, each repaired by the same inpainter (\method without preference
% tuning), on the 7 clips that carry dataset labels. A dot is one clip, and black marks the mean with its 95\% confidence
% interval (SUREAL MOS from eleven observers). The mean rating of our regions lies between those of the dataset
% annotation and the Qwen2.5-VL-72B + SAM3 regions, and the repairs from all three are rated alike for fixing and
% preservation. None of the differences on these 7 clips is significant after Holm correction.}
\caption{Ratings of the three localizations on the 7 annotated clips, each repaired by \method without preference tuning (dots are clips, black is the mean with its 95\% CI). The mean rating of our regions lies between those of the dataset annotation and the 72B pipeline, and no difference on these 7 clips is significant after Holm correction.}
\label{fig:mosloc}
\end{figure*}


==> figures/fig_pair_blocks.tex <==
% Graphic in figures/assets/, made by the study session (rating-app/analysis/pair_paper_figs.py).
\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/assets/fig_pair_blocks.pdf}
\caption{The two control blocks of the blind pairwise follow-up. Left: on 15 training clips, the share of answers that prefer the seed with the higher Video Jev score, against the Jev gap between the two seeds of that clip, filled for \emph{fixed} and open for \emph{preserved}. Right: on 10 test clips, the share of answers that prefer the LoRA at rank 32 over rank 16, one dot per clip, with the pooled share and its 95\% binomial interval.}
\label{fig:supp_pair_blocks}
\end{figure}


==> figures/fig_pair_fix_vs_preserve.tex <==
% Graphic in figures/assets/, made by the study session (rating-app/analysis/pair_paper_figs.py).
\begin{figure}[t]
\centering
\includegraphics[width=0.78\linewidth]{figures/assets/fig_pair_fix_vs_preserve.pdf}
\caption{Blind pairwise follow-up: fixing (x, JOD, 0 = the unrepaired original) against preservation (y, JOD, 0 = \method) per repair, pwcmp scale from six observers with 95\% bootstrap confidence intervals over observers. Circles edit a region and squares regenerate the whole video. Small dots are the per-clip scores of each repair (30 clips, posterior per clip), drawn along the line through its pooled score. Only \method lies to the right of the original on fixing.}
\label{fig:supp_pair_fixpreserve}
\end{figure}


==> figures/fig_pair_per_clip.tex <==
% Graphic in figures/assets/, made by the study session (rating-app/analysis/pair_paper_figs.py).
\begin{figure*}[t]
\centering
\includegraphics[width=0.92\linewidth]{figures/assets/fig_pair_per_clip.pdf}
\caption{Blind pairwise follow-up, per clip: the posterior scale of the three repairs on each of the 30 clips for \emph{fixed} (left, 0 = the unrepaired original) and \emph{preserved} (right, 0 = \method), clips sorted by the \method fixing score. Six observers per clip, so the per-clip scores are coarse and shrunk towards 0 by the prior.}
\label{fig:supp_pair_clips}
\end{figure*}


==> figures/fig_pair_win_matrix.tex <==
% Graphic in figures/assets/, made by the study session (rating-app/analysis/pair_paper_figs.py).
\begin{figure*}[t]
\centering
\includegraphics[width=0.86\linewidth]{figures/assets/fig_pair_win_matrix.pdf}
\caption{Blind pairwise follow-up: share of direct trials in which the row repair was preferred over the column repair, for \emph{fixed} (left, 180 blind trials per pair of repairs and 60 anchor trials per repair against the original) and \emph{preserved} (right, blind trials only). The small number is the pwcmp JOD difference, bold marks a two-tailed $p<0.05$ from the bootstrap over observers.}
\label{fig:supp_pair_wins}
\end{figure*}


==> figures/supp_block_fn.tex <==
% Negative (where our region misses part of the annotated artifact), added on the owner's request (11-22).
% Self-contained, comment out its \input line to drop it. Graphic: artifact_pipeline/scripts/fig_supp_visuals.py fn
On 7 of the 103 test clips our region covers less than 80\% of the annotated artifact pixels, and \cref{fig:supp_fn} shows the four with the lowest coverage, where the region leaves out part of what the annotation marks.\TODO{Negative result, review: partial misses of the localizer.}

\begin{figure}[t]
\centering
\includegraphics[width=\linewidth]{figures/assets/fig_supp_fn.jpg}
%\caption{The four test clips where our region covers the least of the annotated artifact, at the frame where the most annotated pixels fall outside it. The share of annotated pixels covered by our region is given on each.}
\caption{\textbf{Where our region misses part of the artifact.} The four test clips where our region covers the least of the annotated artifact, at the frame where the most annotated pixels fall outside it. The share of annotated pixels covered by our region is given on each.}
\label{fig:supp_fn}
\end{figure}


==> tables/s1_partial.tex <==
% generated by artifact_pipeline/scripts/paper_tables.py — do not edit by hand
\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{3pt}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccccr}
\toprule
Variant & Judge $\Delta\downarrow$ & DINOv2$\uparrow$ & CLIP$\uparrow$ & LPIPS$\downarrow$ & s/clip \\
\midrule
full redraw (\method) & +0.21 & 0.907 & 0.938 & 0.131 & 73 \\
partial redraw 0.85 & +0.23 & 0.863 & 0.906 & 0.133 & 56 \\
partial redraw 0.7 & -0.03 & 0.919 & 0.936 & 0.096 & 46 \\
partial redraw 0.5 & -0.11 & 0.945 & 0.955 & 0.071 & 37 \\
\bottomrule
\end{tabular}}
\caption{Redraw strength inside the region, on the 103 test clips with the teacher's regions. Partial redraw starts from the original noised to the given strength, without a reference image. Lower strengths score better on every automatic measure, but none of these measures tells whether the artifact is gone (see text).}
\label{tab:supp_partial}
\end{table}


==> tables/s2_stimuli.tex <==
% generated by artifact_pipeline/scripts/supp_tables.py — do not edit by hand
\begin{table*}[t]
\centering\small
\begin{tabular}{llllp{0.42\textwidth}}
\toprule
Clip & Source & Generator & fps & Artifact (72B description) or generation prompt \\
\midrule
gen\_cogx2\_113 & example pool & CogVideoX-2B & 8 & prompt: kids playing on a playground with swings and a slide, realistic video \\
gen3\_00162 & BrokenVideos test & Gen-3 & 24 & character floating mid-air \\
gen\_wan22\_095 & example pool & Wan2.2-A14B & 16 & prompt: a monkey swinging between tree branches, realistic video \\
gen\_cogx2\_005 & example pool & CogVideoX-2B & 8 & prompt: a person typing quickly on a laptop keyboard in a cafe, realistic video \\
Cog5B\_00068 & BrokenVideos test & CogVideoX-5B & 8 & The microwave door appears to open unnaturally; The sandwich seems to change position abruptly \\
Cog5B\_00181 & BrokenVideos test & CogVideoX-5B & 8 & distorted facial features of the robot; inconsistent lighting on the person's face \\
Cog5B\_00030 & BrokenVideos test & CogVideoX-5B & 8 & distorted body parts; floating bucket \\
Cog5B\_00653 & BrokenVideos test & CogVideoX-5B & 8 & artifacts around the woman's body \\
OpenSora1.2\_00224 & BrokenVideos test & Open-Sora 1.2 & 24 & distorted body parts \\
gen3\_00109 & BrokenVideos test & Gen-3 & 24 & hand appears distorted near the oven handle \\
\bottomrule
\end{tabular}
\caption{The ten clips of the perceptual study, drawn at random from the clips with a Gemini Omni repair. Example-pool clips carry no labels, so the artifact column gives their generation prompt.}
\label{tab:supp_stimuli}
\end{table*}


==> tables/s7_categories.tex <==
% generated by artifact_pipeline/scripts/artifact_categories.py
\begin{table}[t]
\centering\footnotesize
\setlength{\tabcolsep}{2.5pt}
\begin{tabular}{lrcccc}
\toprule
Class & Clips & Coverage$\uparrow$ & Area & DINOv2$\uparrow$ & LPIPS$\downarrow$ \\
\midrule
Biological motion and anatomy & 68 & 99\% & 35\% & 0.906 & 0.127 \\
Object permanence and morphing & 43 & 95\% & 33\% & 0.904 & 0.108 \\
Temporal flicker and texture & 24 & 96\% & 36\% & 0.932 & 0.127 \\
Physical dynamics & 23 & 97\% & 30\% & 0.889 & 0.118 \\
\bottomrule
\end{tabular}
\caption{\method by artifact class on the 103 test clips. A clip counts in every class its artifacts belong to, from the teacher's description of each violation. Coverage is the share of annotated artifact pixels inside our region, Area its share of the frame, and DINOv2 and LPIPS compare the repair with the input.}
\label{tab:supp_categories}
\end{table}


==> tables/s8_pairwise.tex <==
% generated from rating-app/analysis/pair_paper_figs.py (analysis_out_pair/paper/tab_pair_results.tex), Nov 21 2026
\begin{table*}[t]
\centering\small
\setlength{\tabcolsep}{5pt}
\begin{tabular}{llrrr}
\toprule
Question & Condition & JOD & 95\% CI & Comparisons \\
\midrule
Fixed & Original (no repair) & 0 & -- & 180 \\
 & \method & +0.85 & [+0.51, +1.29] & 420 \\
 & Omni 1.1 Flash & +0.15 & [$-$0.12, +0.40] & 420 \\
 & Wan2.2 & $-$0.07 & [$-$0.67, +0.33] & 420 \\
\midrule
Preserved & \method & 0 & -- & 360 \\
 & Omni 1.1 Flash & $-$0.33 & [$-$0.66, $-$0.03] & 360 \\
 & Wan2.2 & $-$2.34 & [$-$2.73, $-$2.00] & 360 \\
\bottomrule
\end{tabular}
\hspace{1.5em}
\begin{tabular}{llrrrrr}
\toprule
Question & Contrast & $\Delta$JOD & 95\% CI & Direct wins & Clips & $p$ \\
\midrule
Fixed & \method vs.\ Omni 1.1 Flash & +0.70 & [+0.36, +1.15] & 124/180 (69\%) & 18/6/6 & .002 \\
 & \method vs.\ Wan2.2 & +0.92 & [+0.26, +1.80] & 126/180 (70\%) & 19/3/8 & .041 \\
 & Omni 1.1 Flash vs.\ Wan2.2 & +0.22 & [$-$0.17, +0.71] & 107/180 (59\%) & 14/9/7 & .347 \\
 & \method vs.\ original & +0.85 & [+0.51, +1.29] & 48/60 (80\%) & 8/1/1 & $<$.001 \\
 & Omni 1.1 Flash vs.\ original & +0.15 & [$-$0.12, +0.40] & 27/60 (45\%) & 4/5/1 & .594 \\
 & Wan2.2 vs.\ original & $-$0.07 & [$-$0.67, +0.33] & 29/60 (48\%) & 5/4/1 & .786 \\
\midrule
Preserved & \method vs.\ Omni 1.1 Flash & +0.33 & [+0.03, +0.66] & 104/180 (58\%) & 16/11/3 & .045 \\
 & \method vs.\ Wan2.2 & +2.34 & [+2.00, +2.73] & 171/180 (95\%) & 29/1/0 & $<$.001 \\
 & Omni 1.1 Flash vs.\ Wan2.2 & +2.01 & [+1.84, +2.25] & 163/180 (91\%) & 29/1/0 & $<$.001 \\
\bottomrule
\end{tabular}
\caption{Blind pairwise follow-up, six observers and 30 clips. Left: pwcmp JOD scale with 95\% bootstrap confidence intervals over observers, 0 is the unrepaired original for \emph{fixed} and \method for \emph{preserved}. Right: pairwise differences, the share of direct trials won by the first method, the number of clips whose majority preferred it (won/lost/tied), and the two-tailed $p$ from the bootstrap covariance, Holm-adjusted over the three repair contrasts of each question and, separately, over the three anchor contrasts.}
\label{tab:supp_pairwise}
\end{table*}


==> tables/t3_localization.tex <==
% generated by artifact_pipeline/scripts/paper_tables.py — do not edit by hand
\begin{table}[t]
\centering\small
\setlength{\tabcolsep}{1.8pt}
\begin{tabular}{lrrcccc}
\toprule
Localizer & Params & s/clip & J\&F$\uparrow$ & Area & Judge $\Delta\downarrow$ & Localize$\uparrow$ \\
\midrule
BrokenVideos & -- & -- & -- & 12\% & +0.38 & 3.94{\scriptsize$\pm$1.16} \\
\midrule
VLM + SAM3 & 72B & $\sim$140 & \textbf{0.15} & 31\% & +0.48 & 3.26{\scriptsize$\pm$0.97} \\
\textbf{\method} & 45M & 1.3 & 0.13 & 33\% & \textbf{+0.30} & \textbf{3.63}{\scriptsize$\pm$0.80} \\
\bottomrule
\end{tabular}
% \caption{Localizers of the perceptual study. Every region feeds the same inpainter (\method without preference tuning). J\&F is the DAVIS region and boundary score against the BrokenVideos masks, Area the share of the frame inside the region, and Judge $\Delta$ the VLM judge change after repair on the 103 test clips. Localize is the observers' localization MOS recovered with SUREAL on the 7 study clips with dataset labels, $\pm$ half the 95\% CI. BrokenVideos is the oracle, its dataset annotation widened by 24 pixels, and VLM + SAM3 plans the repair with Qwen2.5-VL-72B and segments the named objects with SAM3, its time including the VLM. All localizers we compared are in the supplementary material. Best values in bold.}
\caption{Localizers of the perceptual study, each repaired by \method without preference tuning. J\&F is against the BrokenVideos masks, Area is the share of the frame, Judge $\Delta$ is on the 103 test clips, and Localize is the observer MOS on the 7 annotated study clips $\pm$ half the 95\% CI. BrokenVideos is the annotation widened by 24 pixels, and VLM + SAM3 uses Qwen2.5-VL-72B, its time including the VLM. All localizers are in the supplementary material.}
\label{tab:localization}
\end{table}

